SIR-DIFF: Sparse Image Sets Restoration with Multi-View Diffusion Model

The computer vision community has developed numerous techniques for digitally restoring true scene information from single-view degraded photographs, an important yet extremely ill-posed task. In this work, we tackle image restoration from a different perspective by jointly denoising multiple photographs of the same scene. Our core hypothesis is that degraded images capturing a shared scene contain complementary information that, when combined, better constrains the restoration problem. To this end, we implement a powerful multi-view diffusion model that jointly generates uncorrupted views by extracting rich information from multi-view relationships. Our experiments show that our multi-view approach outperforms existing single-view image and even video-based methods on image deblurring and super-resolution tasks. Critically, our model is trained to output 3D consistent images, making it a promising tool for applications requiring robust multi-view integration, such as 3D reconstruction or pose estimation.

==> tbl/1_quantitative_deblur.tex <==

\begin{table*}[t]
\centering
\label{tab:deblurring_table}
% \vspace{0.15cm}
\caption{
    \textbf{Quantitative Comparisons on Different Image and Video Motion Deblurring benchmarks.} 
    The best is \textbf{highlighted} and the second best is \underline{underlined}.
}
\vspace{-0.3cm}
\resizebox{0.8\textwidth}{!}{
\huge
\begin{tabular}{clccccccccc}
\cmidrule[\heavyrulewidth]{2-11}
 & \textbf{Dataset}
 & \multicolumn{3}{c}{\textbf{Scannet++}~\cite{yeshwanth2023scannet++}} & \multicolumn{3}{c}{\textbf{ETH3D}~\cite{schops2019bad}} & \multicolumn{3}{c}{\textbf{CO3D}~\cite{reizenstein2021common}} \\
 & Method & FID $\downarrow$ & LPIPS $\downarrow$ & Consis.$\downarrow$ & FID $\downarrow$ & LPIPS $\downarrow$ & Consis.$\downarrow$ & FID $\downarrow$ & LPIPS $\downarrow$ & Consis.$\downarrow$ \\ \cmidrule{2-11}
& PromptIR~\cite{potlapalli2024promptir} &  81.28 & 0.248 & - & 150.34 & 0.537 & - & 166.3 & \underline{0.350} & -  \\

& Restromer~\cite{zamir2022restormer}  & \underline{49.72} & \underline{0.232} & - & \underline{73.47} & \underline{0.330} & - & 144.8 & 0.426 & -  \\
& VRT~\cite{liang2024vrt}  & 134.5 & 0.371 & - & 160.4 & 0.530 & - & 170.4 & 0.440 & - \\  
& \textbf{1 Frame Ours}  & 81.58 & 0.247 & - & 109.6 & 0.350 & - & \underline{137.9} & 0.357 & - \\     
& \textbf{Ours}   & \textbf{40.09} & \textbf{0.160} & - & \textbf{67.31} & \textbf{0.263} & - & \textbf{85.67} & \textbf{0.275} & -
  
  \\ \cmidrule{2-11}

\end{tabular}
}
\vspace{-0.35cm}
\end{table*}

==> tbl/1_quantitative_sr.tex <==
\begin{table*}[t]
\centering
\label{tab:sr_table}
% \vspace{-0.15cm}
\caption{\textbf{
        Quantitative comparisons on different Image and Video SR 
        benchmarks.} 
        The best is \textbf{highlighted} and the second best is \underline{underlined}.
        }
% \vspace{-0.3cm}
\resizebox{0.9\textwidth}{!}{%
\huge
\begin{tabular}{clcccccccccccc}
\cmidrule[\heavyrulewidth]{2-14}
 & \textbf{Dataset}
 & \multicolumn{4}{c}{\textbf{Scannet++}~\cite{yeshwanth2023scannet++}} & \multicolumn{4}{c}{\textbf{ETH3D}~\cite{schops2019bad}} & \multicolumn{4}{c}{\textbf{CO3D}~\cite{reizenstein2021common}} \\
 
 & Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Consis.$\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Consis.$\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Consis.$\downarrow$ \\ \cmidrule{2-14}

& SAMDiff~\cite{wang2024sam} & 24.13 & 0.216 & 0.758 & - & 19.16 & 0.317 & 0.495 & - & 23.90 & 0.246 & 0.626& -  \\
& OSEDiff~\cite{wu2024one} & 25.22 & \underline{0.808} & \underline{0.154} & - & 21.93 & \textbf{0.621} & 0.264 & - & \underline{24.50} & \textbf{0.658} & \underline{0.277} & -  \\
& UAV~\cite{zhou2024upscale}  & 23.23 & 0.677 & 0.354 & - & 20.39 & 0.506 & 0.413 & - & 22.73 & 0.566 & 0.400 & -\\  
& \textbf{1 Frame Ours}   & \underline{25.85} & 0.792 & 0.164 & - & \underline{21.97} & 0.593 & \underline{0.221} & - & 24.35 & 0.641 & 0.301 & - \\     
& \textbf{Ours}   & \textbf{27.38} & \textbf{0.837} & \textbf{0.099} & - & \textbf{22.58} & \textbf{0.621} & \textbf{0.201} & - & \textbf{24.53} & \textbf{0.658} & \textbf{0.210} & -
  
  \\ \cmidrule{2-14}

\end{tabular}
}
% \vspace{-0.4cm}
\label{tab:main_table}
\end{table*}
